Order-Embeddings of Images and Language

Hypernymy, textual entailment, and image captioning can be seen as special cases of a single visual-semantic hierarchy over words, sentences, and images. In this paper we advocate for explicitly modeling the partial order structure of this hierarchy. Towards this goal, we introduce a general method for learning ordered representations, and show how it can be applied to a variety of tasks involving images and language. We show that the resulting representations improve performance over current approaches for hypernym prediction and image-caption retrieval.

==> related_work.tex <==
(The following is moved from Ryan's alternative introduction, to be used as part of a broader related work section for caption-image retrieval)

Multimodal embedding methods that map images and words [?] or images and sentences [?] into a common vector space provide a natural framework for relating these two modalities. These methods not only provide a way of annotating images with lingual descriptions [?] but also allow for improved learning of word representations through visual grounding [?]. Words are typically represented as distributed representations [?] and images are mapped through a pre-trained deep convolutional network [?]. In the case of sentences, both LSTM [?] and convolutional networks [?] have demonstrated strong performance as compositional functions of word representations [?]. 

The {\color{red}visual} semantic hierarchy utilizes an asymmetrical notion of similarity. For example,  the similarity between "woman skiing" and "woman" is not the same as "woman" and "woman skiing". {\color{red} this has nothing to do with "visual", this is just semantics" This is a comment of why I put "visual" in red before}
This is because while all women who ski are women, not all images of women depict women skiing. Despite this fact, almost all multimodal embedding methods utilize a symmetric notion of similarity, often via cosine similarity integrated into CCA [?] {\color{red} why are you saying integrated into CCA? Isn't talking about cosine enough?} or a pairwise ranking loss [?]. {\color{red} you said almost all. Then what is the exception?}
This is very limiting, and current multimodal embeddings cannot learn the inherently hierarchical structure of visual-semantic concepts. 
A symmetric similarity cannot capture that asymmetric structure of the visual-semantic hierarchy and thus existing multimodal embedding methods cannot readily learn this hierarchical structure. 

In contrast, in this work we propose  to use an  asymmetric similarity that  captures the partial ordering of the visual-semantic hierarchy. 
In this work, we target this weakness of existing embedding methods by replacing a symmetric similarity with an asymmetric one that captures the partial ordering of a semantic hierarchy. 
Our contribution can easily be integrated into any existing embedding method by replacing the existing comparison operation with ours. 

